MCGAN: Enhancing GAN Training with Regression-Based Generator Loss

Generative adversarial networks (GANs) have emerged as a powerful tool for generating high-fidelity data. However, the main bottleneck of existing approaches is the lack of supervision on the generator training, which often results in undamped oscillation and unsatisfactory performance. To address this issue, we propose an algorithm called Monte Carlo GAN (MCGAN). This approach, utilizing an innovative generative loss function, termly the regression loss, reformulates the generator training as a regression task and enables the generator training by minimizing the mean squared error between the discriminator's output of real data and the expected discriminator of fake data. We demonstrate the desirable analytic properties of the regression loss, including discriminability and optimality, and show that our method requires a weaker condition on the discriminator for effective generator training. These properties justify the strength of this approach to improve the training stability while retaining the optimality of GAN by leveraging strong supervision of the regression loss. Extensive experiments on diverse datasets, including image data (CIFAR-10/100, FFHQ256, ImageNet, and LSUN Bedroom), time series data (VAR and stock data) and video data, are conducted to demonstrate the flexibility and effectiveness of our proposed MCGAN. Numerical results show that the proposed MCGAN is versatile in enhancing a variety of backbone GAN models and achieves consistent and significant improvement in terms of quality, accuracy, training stability, and learned latent space.

==> Figures/CIFAR10/CIFAR10_BigGAN.tex <==
\newcolumntype{Y}{>{\centering\arraybackslash}X}
\begin{table}[!ht]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabularx}{1.4\textwidth}{l| Y || Y || Y  || Y}
\toprule
\multicolumn{1}{l|}{Metrics} & \multicolumn{1}{c||}{ IS} &   \multicolumn{1}{c||}{FID}& 
 \multicolumn{1}{c||}{$\text{F}_{0.125}$} & \multicolumn{1}{c}{$\text{F}_{0.8}$}    
\\\midrule
SNGAN   & 8.67  & 13.33 & 0.985 & 0.976  \\\midrule
BigGAN   & 9.81 & 8.08  & 0.993  & 0.992  \\\midrule
ReACGAN   & 9.89   &  7.88   & 0.994  & 0.992 \\\midrule
MCWGAN     & \textbf{10.04}   & \textbf{6.41}  & -    & - 
 \\\bottomrule
\end{tabularx}}
\caption{Comparison with SOTA classider-based GANs and projetion-based GANs with BigGAN as the backbone on CIFAR-10 datsets using IS, FID, $\text{F}_{0.125}$, $\text{F}_{0.8}$.}\label{table_CIFAR10_TBD}
\end{table}


==> Figures/CIFAR10/CIFAR10_DiffAug_copy.tex <==
\newcolumntype{Y}{>{\centering\arraybackslash}X}
\begin{table}[!ht]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabularx}{1.4\textwidth}{l| Y || Y}
\toprule
\multicolumn{1}{l|}{Metrics} & \multicolumn{1}{c||}{IS} &   \multicolumn{1}{c}{FID}   
\\\midrule
Hinge   & 9.232$\pm$ 0.14 & 6.10  \\\midrule
+DiffAug   & 9.45$\pm $  0.06 &  4.69   \\\midrule
+MC   & 9.66 $\pm$ 0.09   &  5.28  \\\midrule
+MC+DiffAug     & \textbf{10.04 $\pm$ 0.10} &  \textbf{3.72}
 \\\bottomrule
\end{tabularx}}
\caption{Comparison between Differential Augmentation and MC method using BigGAN as the backbone on CIFAR-10 datasets. IS and FID are measured using 50K samples}\label{table_CIFAR10}
\end{table}


==> Figures/CIFAR10/CIFAR10_DiffAug_finetune.tex <==
\begin{table}[!ht]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabularx}{1.4\textwidth}{|l| Y|Y| Y|}
\toprule
\multicolumn{1}{|l|}{Loss} & \multicolumn{3}{c|}{Hinge}    
\\\midrule
\multicolumn{1}{|l|}{Metrics} & \multicolumn{1}{c|}{IS} &   \multicolumn{1}{c|}{FID} &
\multicolumn{1}{c|}{IFID}
\\\midrule
Original  & 9.41 $\pm$ 0.11 & 5.02 & 16.20 
\\\midrule 
+DiffAug   & 9.57 $\pm $  0.06 &  3.688 & 13.51
\\\midrule
+MC+DiffAug  & 9.93 $\pm$ 0.12 &  \textbf{3.55} & 13.75
 \\\bottomrule
\end{tabularx}}
\caption{Comparison between Differential Augmentation and MC method using fine-tuned Big-ResNet as the backbone on CIFAR-10 datasets. IS and FID are measured using 50K samples}\label{table_CIFAR10_finetune}
\end{table}


==> Figures/CIFAR10/CIFAR10_Loss.tex <==
\newcolumntype{Y}{>{\centering\arraybackslash}X}
\begin{table}[!ht]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabularx}{1.4\textwidth}{l| Y || Y || Y  || Y}
\toprule
\multicolumn{1}{l|}{Metrics} & \multicolumn{1}{c||}{ IS} &   \multicolumn{1}{c||}{FID}& 
 \multicolumn{1}{c||}{$\text{F}_{0.125}$} & \multicolumn{1}{c}{$\text{F}_{0.8}$}    
\\\midrule
Hinge   & 9.21 & 8.36 & -    & -   \\
+MC   & \textbf{9.66} & \textbf{5.28} & -    & -   \\\midrule
Non-saturating   & 9.30  & 8.17  & -    & -   \\
+MC   & \textbf{9.92}    & \textbf{6.78}  & -    & -   \\\midrule
Omni   & 9.79 & 5.57  & -    & -  \\
+MC   & 9.35 & 6.32 & -    & -  \\\midrule
ReACGAN     & 9.89   & 7.88  & -    & - \\
+MC     & -  & -  & -    & - 
 \\\bottomrule
\end{tabularx}}
\caption{Comparison with different discriminative loss with BigGAN as the backbone on CIFAR-10 datsets using IS, FID, $\text{F}_{0.125}$, $\text{F}_{0.8}$.}\label{table_CIFAR10_TBD}
\end{table}


==> Figures/CIFAR10/CIFAR10_StyleGAN2.tex <==
%\newcolumntype{Y}{>{\centering\arraybackslash}X}
\begin{table}[!ht]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabularx}{0.7\textwidth}{l| Y|Y| Y||Y|Y|Y}
\toprule
    \multicolumn{1}{l|}{Loss} & \multicolumn{3}{c||}{Hinge} &   \multicolumn{3}{c}{BCE}   
\\\midrule
\multicolumn{1}{l|}{Metrics} & \multicolumn{1}{c|}{IS $\uparrow$} &   \multicolumn{1}{c|}{FID $\downarrow$} &
\multicolumn{1}{c||}{IFID $\downarrow$}&
\multicolumn{1}{c|}{IS $\uparrow$} &   \multicolumn{1}{c|}{FID $\downarrow$} & \multicolumn{1}{c}{IFID $\downarrow$}
\\\midrule
StyleGAN2+DiffAug   & 10.1859 &  2.2475& 11.4037& 10.0281&  2.4387& 11.6191
\\
\quad\quad\quad+MC+DiffAug  & \textbf{10.2608} & \textbf{2.1650} & \textbf{11.0351} & \textbf{10.0995} &\textbf{2.3595} & \textbf{11.3004}
 \\\midrule
  StyleGAN2+ADA  & 10.53  & 2.31 &  11.82 &  -  & - & -
 \\\bottomrule
\end{tabularx}}
\caption{Quantitative results of image generation on CIFAR-10 using cStyleGAN2 w/o and with our MC method and Differentiable Augmentation.}\label{table_CIFAR-10_stylegan2}
\end{table}


==> Figures/CIFAR100/CIFAR100_BigGAN_copy.tex <==
\newcolumntype{Y}{>{\centering\arraybackslash}X}
\begin{table}[!ht]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabularx}{1.4\textwidth}{l| Y || Y }
\toprule
\multicolumn{1}{l|}{Metrics} & \multicolumn{1}{c||}{ IS} &   \multicolumn{1}{c}{FID}
\\\midrule
BigGAN   &  9.98  & 13.73 \\\midrule
OmniGAN   & \textbf{13.30} & 8.41  \\\midrule
ReACGAN   & -   &  -   \\\midrule
MCGAN     & 11.32   & \textbf{7.70}  
 \\\bottomrule
\end{tabularx}}
\caption{Comparison with SOTA classider-based GANs and projetion-based GANs with BigGAN as the backbone on CIFAR-100   datsets using IS, FID.}\label{table_CIFAR10_aux}
\end{table}


==> Figures/Timeseries/MCGAN/ARCH/table_arch.tex <==
\begin{table}[!ht]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabularx}{1.4\textwidth}{l| c || c || c || c || c}
\toprule
Metrics & abs metric &  acf score & 
correlation &
$R^2(\%)$ & Sig-$W_1$    
\\\midrule
SigCWGAN   & 0.01730, {0.01674}  & 0.01342, \textbf{0.01192}     & \textbf{0.01079}, \textbf{0.07435} &2.996, {7.948}   & \textbf{0.18448}, \textbf{4.36744}                \\\midrule
TimeGAN   & 0.02155, 0.02127    & 0.05792, 0.03035     & {0.12363}, {0.61488} & 5.955, 8.586 & 0.58541, 5.99482\\\midrule
RCGAN     & 0.02094, \textbf{0.01655}   & 0.03362, 0.04075     & 0.04606, 0.15353     & \textbf{2.788}, \textbf{7.190}  & 0.47107, 5.43254                   \\\midrule
GMMN      & \textbf{0.01608}, 0.02387   & \textbf{0,01283}, 0.02676  & 0.04651, 0.22380   & 9.049, 7.384 & 0.59073, 6.23777    \\\bottomrule
\end{tabularx}
}
\caption{Numerical results of the ARCH datasets. We use the relative error of TSTR $R^{2}$ against TRTR  $R^{2}$ as the $R^2$ metric.}
\label{table_stocks_reshape}
\end{table}

==> Figures/Timeseries/MCGAN/STOCK/CoverageRatioTest.tex <==
\begin{table}[!ht]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabularx}{0.75\textwidth}{l| c || c }
\toprule
Models & Ratio of 1-day ahead returns &  Ratio of 5-day ahead returns
\\\midrule
SigCWGAN& 8.04\%, 9.11\% &3.62\%,\textbf{4.02}\%\\\midrule
MCGAN& 4.29\%, 4.29\% & 3.35\%,\textbf{4.02}\%\\\midrule
TimeGAN& 6.70\%, 8.31\% & \textbf{5.63\%},6.70\%\\\midrule
RCGAN&\textbf{4.95\%},\textbf{4,42\%} &3.62\%,3.88\%\\\midrule
GMMN& 6.70\%,6.70\%& 6.43\%,6.30\%\\\midrule
GARCH&9.70\%,8.75\% &7.63\%,6.70\%\\\bottomrule
\end{tabularx}
}
\caption{Results of coverage ratio test applied to SPX and DJI stock returns. In each cell, the left/right numbers are the results for the SPX/ DJI data respectively. A ratio that is closer to $5\%$ indicates a more accurate 95\% VaR estimate. The VaR estimate of each model for each observation is obtained using 5000 generated samples.}
\label{table_stocks_coverageratio_mcgan}
\end{table}

==> Figures/Timeseries/MCGAN/STOCK/table_stock.tex <==
\begin{table}[ ht]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabularx}{0.8\textwidth}{c| l| Y | Y| Y| Y}
\toprule
 \multicolumn{1}{c|}{Loss}&\multicolumn{1}{l|}{Method} & \multicolumn{1}{c|}{ABS $\downarrow$} &   \multicolumn{1}{c|}{Corr $\downarrow$} &
\multicolumn{1}{c|}{ACF $\downarrow$}&
\multicolumn{1}{c|}{ACF($|x|$)$\downarrow$} &
\multicolumn{1}{c}{ACF($x^2$) $\downarrow$}
\\\midrule
 \multirow{2}{*}{Hinge} & original  & 0.01201 & 0.33790 & 0.25747 & 0.25818 & 0.30180  \\
&\quad +MC   & \textbf{0.01059} & \textbf{0.06233} & \textbf{0.14803} & \textbf{0.09510}&\textbf{0.08645}
 \\\midrule
 \multirow{2}{*}{BCE} &original  & \textbf{0.01022} & 0.13747 &  0.18711  & 0.14553 & 0.13348 
\\
&\quad +MC  & 0.01286 &  \textbf{0.063744} & \textbf{0.10474} &  \textbf{0.07496}& \textbf{0.07048}
 \\\bottomrule
\end{tabularx}}
\caption{Quantitative results of time-series generation on SPX/DJI data using RNN w/o and with our MC method.}\label{table_stock_loss}
\end{table}

==> Figures/Timeseries/MCGAN/VAR/table_var.tex <==
\begin{table}[!ht]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabularx}{1.4\textwidth}{l| c || c || c || c || c}
\toprule
Metrics & abs metric &  acf metric & 
correlation &
$R^2(\%)$ & Sig-$W_1$    
\\\midrule
SigCWGAN   & 0.01730, {0.01674}  & 0.01342, \textbf{0.01192}     & \textbf{0.01079}, \textbf{0.07435} &2.996, {7.948}   & \textbf{0.18448}, \textbf{4.36744}                \\\midrule
TimeGAN   & 0.02155, 0.02127    & 0.05792, 0.03035     & {0.12363}, {0.61488} & 5.955, 8.586 & 0.58541, 5.99482\\\midrule
RCGAN     & 0.02094, \textbf{0.01655}   & 0.03362, 0.04075     & 0.04606, 0.15353     & \textbf{2.788}, \textbf{7.190}  & 0.47107, 5.43254                   \\\midrule
GMMN      & \textbf{0.01608}, 0.02387   & \textbf{0,01283}, 0.02676  & 0.04651, 0.22380   & 9.049, 7.384 & 0.59073, 6.23777    \\\bottomrule
\end{tabularx}
}
\caption{Numerical results of the VAR datasets. We use the relative error of TSTR $R^{2}$ against TRTR  $R^{2}$ as the $R^2$ metric.}
\label{table_stocks_reshape}
\end{table}

==> numerical_results/BigGAN_CIFAR10_trainingtime.tex <==
\begin{table}[!ht]
\caption{Training time (seconds) for 5k iterations.}
\centering
\resizebox{\linewidth}{!}{
\begin{tabularx}{0.65\textwidth}{l|Y|Y|Y|Y|Y}
\hline
\textbf{Method} & \textbf{w/o MC} & \textbf{M=5} & \textbf{M=10} & \textbf{M=15} & \textbf{M=20} \\ \hline
\textbf{Time (s)} & 976 & 1560 & 2171 & 2868 & 3498 \\ \hline
\end{tabularx}
}
\label{tab:training_time}
\end{table}


==> numerical_results/table_arch.tex <==
\begin{table}[!ht]
\caption{Numerical results of the ARCH(k) datasets.}\label{table_arch}
\centering 
\begin{tabularx}{.7\textwidth}{l|Y || Y|| Y}
\toprule
Settings & \multicolumn{1}{c||}{$k=2$} & \multicolumn{1}{c||}{$k=3$} & \multicolumn{1}{c}  {$k=4$}\\ \midrule
\multicolumn{4}{c}{Metric on marginal distribution}                 \\\midrule
SigCWGAN&0.01956&0.00884&0.01342\\
MCGAN&\textbf{0.00883}&\textbf{0.00489}&\textbf{0.00638}\\
TimeGAN&0.01712&0.01501&0.01239\\
RCGAN&0.01249&0.01113&0.00814\\
GMMN&0.02079&0.01498&0.00980\\
\midrule
\multicolumn{4}{c}{Absolute difference of lag-1 autocorrelation}                            \\\midrule
SigCWGAN&\textbf{0.01178}&\textbf{0.00601}&0.00687\\
MCGAN&0.05063&0.05070&\textbf{0.00647}\\
TimeGAN&0.06774&0.04640&0.00788\\
RCGAN&0.03317&0.02608&0.02679\\
GMMN&0.02131&0.01270&0.00943\\
\midrule
\multicolumn{4}{c}{$l_1$-norm of real and generated cross correlation matrices}                               \\\midrule
SigCWGAN&0.01002&0.00991&\textbf{0.02645}\\
MCGAN&0.04777&0.03374&0.05829\\
TimeGAN&\textbf{0.00243}&0.01321&0.12278\\
RCGAN&0.00674&\textbf{0.00775}&0.02941\\
GMMN&0.04594&0.05310&0.03074\\
\midrule
\multicolumn{4}{c}{Relative error (\%) of $R^2$ obtained from TSTR. }                   \\\midrule
SigCWGAN&\textbf{0.42229}&\textbf{0.22901}&\textbf{0.51255}\\
MCGAN&1.66906&2.41386&3.53569\\
TimeGAN&7.99938&2.28691&11.3179\\
RCGAN&6.30669&7.65128&5.68634\\
GMMN&77.6923&26.9197&20.6545\\
\midrule
\multicolumn{4}{c}{Sig-$W_1$ distance}                                          \\\midrule
SigCWGAN&\textbf{2.78657}&\textbf{4.25746}&\textbf{7.10808}\\
MCGAN&2.80282&4.27829&7.11126\\
TimeGAN&2.83394&4.29551&7.12979\\
RCGAN&2.80822&4.27600&7.11534\\
GMMN&2.85250&4.30627&7.14542\\
\bottomrule
\end{tabularx}
\end{table}

==> numerical_results/table_stock_reshape.tex <==
%previous table 
%\newcolumntype{Y}{>{\centering\arraybackslash}X}
%\begin{table}[!ht]
%\centering
%\resizebox{\columnwidth}{!}{%
%\begin{tabularx}{1.4\textwidth}{l| Y || Y || Y || Y || Y}
%\toprule
%\multicolumn{1}{l|}{Metrics} & \multicolumn{1}{c||}{marginal %distribution} &   \multicolumn{1}{c||}{auto-correlation}& 
% \multicolumn{1}{c||}{correlation} &
% \multicolumn{1}{c||}{$R^2(\%)$} & \multicolumn{1}{c}{Sig-$W_1$}  %  
%\\\midrule
%SigCWGAN   & 0.01730, {0.01674}  & 0.01342, \textbf{0.01192}     & %\textbf{0.01079}, \textbf{0.07435} &2.996, {7.948}   & %\textbf{0.18448}, \textbf{4.36744}                \\\midrule
%TimeGAN   & 0.02155, 0.02127    & 0.05792, 0.03035     & %{0.12363}, {0.61488} & 5.955, 8.586 & 0.58541, 5.99482\\\midrule
%RCGAN     & 0.02094, \textbf{0.01655}   & 0.03362, 0.04075     & %0.04606, 0.15353     & \textbf{2.788}, \textbf{7.190}  & 0.47107, %5.43254                   \\\midrule
%GMMN      & \textbf{0.01608}, 0.02387   & \textbf{0,01283}, %0.02676  & 0.04651, 0.22380   & 9.049, 7.384 & 0.59073, 6.23777   % \\\bottomrule
%\end{tabularx}}
%\caption{Numerical results of the stock datasets. In each cell, %the left/right number are the result for the SPX data/ the SPX and %DJI data respectively. We use the relative error of TSTR $R^{2}$ %against TRTR  $R^{2}$ as the $R^2$ metric.}
%\label{table_stocks_reshape}
%\end{table}

\newcolumntype{Y}{>{\centering\arraybackslash}X}
\begin{table}[!ht]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabularx}{1.4\textwidth}{l| Y || Y || Y || Y || Y}
\toprule
\multicolumn{1}{l|}{Metrics} & \multicolumn{1}{c||}{marginal distribution} &   \multicolumn{1}{c||}{auto-correlation}& 
 \multicolumn{1}{c||}{correlation} &
 \multicolumn{1}{c||}{$R^2(\%)$} & \multicolumn{1}{c}{Sig-$W_1$}    
\\\midrule
SigCWGAN   & 0.01730, {0.01674}  & 0.01342, \textbf{0.01192}     & \textbf{0.01079}, \textbf{0.07435} &2.996, {7.948}   & \textbf{0.18448}, \textbf{4.36744}                \\\midrule
TimeGAN   & 0.02155, 0.02127    & 0.05792, 0.03035     & {0.12363}, {0.61488} & 5.955, 8.586 & 0.58541, 5.99482\\\midrule
RCGAN     & 0.02094, \textbf{0.01655}   & 0.03362, 0.04075     & 0.04606, 0.15353     & \textbf{2.788}, \textbf{7.190}  & 0.47107, 5.43254                   \\\midrule
GMMN      & 0.01608, 0.02387   & \textbf{0,01283}, 0.02676  & 0.04651, 0.22380   & 9.049, 7.384 & 0.59073, 6.23777   \\\midrule
{\color{red}GARCH}&\textcolor{red}{\textbf{0.01583},0.01670} &\textcolor{red}{0.13392, 0.11337}&\textcolor{red}{0.15791, 0.7290} & \textcolor{red}{12.1253, 12.5686}&\textcolor{red}{0.64825, 6.15344} \\\bottomrule
\end{tabularx}}
\caption{Numerical results of the stock datasets. In each cell, the left/right number are the result for the SPX data/ the SPX and DJI data respectively. We use the relative error of TSTR $R^{2}$ against TRTR  $R^{2}$ as the $R^2$ metric.}
\label{table_stocks_reshape}
\end{table}


==> numerical_results/table_stocks.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \begin{table}[!ht]
% \caption{Numerical results of the stocks datasets.}
% \centering 
% \label{table_stocks}
% \begin{tabularx}{.7\textwidth}{l| c || c}
% \toprule
% Data type & \multicolumn{1}{c||}{SPX} & \multicolumn{1}{c}{SPX + DJI} \\ \midrule
% \multicolumn{3}{c}{Metric on marginal distribution}                 \\\midrule
% SigCWGAN   & 0,01730                 & {0,01674}              \\
% TimeGAN   & 0,02155                 & 0,02127                       \\
% RCGAN     & 0,02094                 & \textbf{0,01655}                       \\
% GMMN      & \textbf{0,01608}        & 0,02387                       \\\midrule
% \multicolumn{3}{c}{Absolute difference of lag-1 autocorrelation}                                           \\\midrule
% SigCWGAN   & {0,01342}                 & \textbf{0,01192}              \\
% TimeGAN   & 0,05792                 & 0,03035                       \\
% RCGAN     & 0,03362                 & 0,04075                       \\
% GMMN      & \textbf{0,01283}        & 0,02676                       \\\midrule
% \multicolumn{3}{c}{$L_1$-norm of real and generated cross correlation matrices}                               \\\midrule
% SigCWGAN   & \textbf{0,01079}        & \textbf{0,07435}              \\
% TimeGAN   & 0,12363                 & 0,61488                       \\
% RCGAN     & 0,04606                 & 0,15353                       \\
% GMMN      & 0,04651                 & 0,22380                       \\\midrule
% \multicolumn{3}{c}{$R^2$ obtained from TSTR. (TRTR first row.)}                   
% \\\midrule
% TRTR      & {0,31706}        & {0,31934}              \\ \midrule
% SigCWGAN   & 0,30797                 & {0,29396}               \\
% TimeGAN   & 0,29818                 & 0,29192                       \\
% RCGAN     & \textbf{0,30822}        & \textbf{0,29638}                       \\
% GMMN      & 0,28837                 & 0,29576                       \\\midrule
% \multicolumn{3}{c}{Sig-$W_1$ distance}                                          \\\midrule
% SigCWGAN   & \textbf{0,31775}        & \textbf{4,36744}              \\
% TimeGAN   & 0,58541                 & 5,99482                       \\
% RCGAN     & 0,47107                 & 5,43254                       \\
% GMMN      & 0,59073                 & 6,23777                       \\ \bottomrule
% \end{tabularx}
% \end{table}
%
%
% Previous Table
%\newcolumntype{Y}{>{\centering\arraybackslash}X}
%\begin{table}[!ht]
%\caption{Numerical results of the stocks datasets.}
%\centering 
%\label{table_stocks}
%\begin{tabularx}{.7\textwidth}{l| Y || Y}
%\toprule
%Data type & \multicolumn{1}{c||}{SPX} & \multicolumn{1}{c}{SPX + %DJI} \\ \midrule
%\multicolumn{3}{c}{Metric on marginal distribution}                 %\\\midrule
%SigCWGAN  & 0.0142 & \textbf{0.0093} \\
%CWGAN  & 0.0111 & 0.0151 \\
%TimeGAN  & 0.0089 & 0.0156 \\
%RCGAN  & \textbf{0.0088} & 0.0140 \\
%GMMN  & 0.0107 & 0.0181 \\ \midrule
%\multicolumn{3}{c}{Absolute difference of lag-1 autocorrelation}    %                                       \\\midrule
%SigCWGAN  & 0.0302 & 0.0447 \\
%CWGAN  & 0.1617 & 0.0571 \\
%TimeGAN  & \textbf{0.0180} & 0.0232 \\
%RCGAN  & 0.0350 & 0.0515 \\
%GMMN  & 0.0273 & \textbf{0.0106} \\ \midrule
%\multicolumn{3}{c}{$L_1$-norm of real and generated cross %correlation matrices}                               \\\midrule
%SigCWGAN  & 0.0503 & \textbf{0.0747} \\
%CWGAN  & \textbf{0.0131} & 0.3908 \\
%TimeGAN  & 0.0793 & 0.5401 \\
%RCGAN  & 0.0654 & 0.3959 \\
%GMMN  & 0.0409 & 0.2103 \\ \midrule
%\multicolumn{3}{c}{$R^2$ obtained from TSTR. (TRTR first row.)}     %              
%\\\midrule
%TRTR      & 0.3689 & 0.3731 \\ \midrule
%SigCWGAN  & \textbf{0.3576} & 0.3466 \\
%CWGAN  & 0.2744 & 0.2694 \\
%TimeGAN  & 0.3551 & \textbf{0.3602} \\
%RCGAN  & 0.3037 & 0.3532 \\
%GMMN  & 0.3375 & 0.3368 \\ \midrule
%\multicolumn{3}{c}{Sig-$W_1$ distance}                              %            \\\midrule
%SigCWGAN  & \textbf{0.0985} & \textbf{0.1307} \\
%CWGAN  & 0.1684 & 0.2881 \\
%TimeGAN  & 0.1265 & 0.2321 \\
%RCGAN  & 0.1462 & 0.2353 \\
%GMMN  & 0.1257 & 0.2448 \\ \bottomrule
%\end{tabularx}
%\end{table}

\newcolumntype{Y}{>{\centering\arraybackslash}X}
\begin{table}[!ht]
\caption{Numerical results of the stocks datasets.}
\centering 
\label{table_stocks}
\resizebox{0.65\columnwidth}{!}{
\begin{tabularx}{.7\textwidth}{l| Y || Y}
\toprule
Data type & \multicolumn{1}{c||}{SPX} & \multicolumn{1}{c}{SPX + DJI} \\ \midrule
\multicolumn{3}{c}{Metric on marginal distribution}                 \\\midrule
SigCWGAN&0.01468&\textbf{0.00879}\\
MCGAN&\textbf{0.00915}&0.00937\\
TimeGAN&0.01064&0.01136\\
RCGAN&0.01134&0.00933\\
GMMN&0.00986&0.01438\\
GARCH&0.01583&0.01670\\
\midrule
\multicolumn{3}{c}{Absolute difference of lag-3 autocorrelation}                                           \\\midrule
SigCWGAN&\textbf{0.02693}&0.03988\\
MCGAN&0.03665&0.03386\\
TimeGAN&0.0341&\textbf{0.03147}\\
RCGAN&0.04192&0.03367\\
GMMN&0.05483&0.06668\\
GARCH&0.05392& 0.05337\\
\midrule
\multicolumn{3}{c}{$L_1$-norm of real and generated cross-correlation matrices}                               \\\midrule
SigCWGAN&\textbf{0.00638}&\textbf{0.10354}\\
MCGAN&0.05641&0.12938\\
TimeGAN&0.0101&0.11342\\
RCGAN&0.0926&0.13699\\
GMMN&0.07498&0.28339\\
GARCH&0.15791&0.72901\\
\midrule
\multicolumn{3}{c}{Relative $R^2$ error (\%). }                   
\\\midrule
SigCWGAN&5.56765&5.28866\\
MCGAN&3.87395&\textbf{4.12438}\\
TimeGAN&8.5833&7.13335\\
RCGAN&\textbf{3.74567}&5.75112\\
GMMN&5.33373&12.17658\\
GARCH&12.1253&12.5686\\
\midrule
\multicolumn{3}{c}{Sig-$W_1$ distance}                                          \\\midrule
SigCWGAN&4.74507&5.18462\\
MCGAN&\textbf{4.73513}&5.19871\\
TimeGAN&4.75276&5.22316\\
RCGAN&4.74362&5.20083\\
GMMN&4.75251&\textbf{5.17637}\\
GARCH&4.75825&5.25344\\
\bottomrule
\end{tabularx}}
\end{table}



==> numerical_results/table_var_dim=3_time.tex <==
%Previous table 
%\newcolumntype{Y}{>{\centering\arraybackslash}X}
%\begin{table}[!ht]
%\caption{Numerical results of $\operatorname{VAR}(1)$ for $d = 3$ %with fixed training time of 2 minutes}\label{table_Var_dim=3_time}
%\centering
%\begin{tabularx}{.55\textwidth}{l| Y}
%\toprule
%\multicolumn{1}{l|}{}     & \multicolumn{1}{c}{Temporal Correlations} % \\ \midrule
%Settings                  & %\multicolumn{1}{c}{$\phi=0.2,\,\,\sigma=0.8$} \\ \midrule
%\multicolumn{2}{c}{Metric on marginal distribution} \\ \midrule
%SigCWGAN  & 0.0314  \\
%CWGAN  & 0.0086  \\
%TimeGAN  & 0.0243  \\
%RCGAN  & 0.0095  \\
%GMMN  & \textbf{0.0084} \\ \midrule
%\multicolumn{2}{c}{Absolute difference of lag-1 autocorrelation} \\ %\midrule
%SigCWGAN  & \textbf{0.0085}  \\
%CWGAN  & 0.0110  \\
%TimeGAN  & 0.0320  \\
%RCGAN  & 0.0332  \\
%GMMN  & 0.0298  \\ \midrule
%\multicolumn{2}{c}{$R^2$ obtained from TSTR. (TRTR first row.)} \\ %\midrule
%\multicolumn{1}{l|}{TRTR} & 0.04197  \\ \midrule
%SigCWGAN  & \textbf{0.0394}  \\
%CWGAN  & 0.0350  \\
%TimeGAN  & 0.0229  \\
%RCGAN  & 0.0214  \\
%GMMN  & 0.0026  \\ \midrule
%\multicolumn{2}{c}{Sig-$W_1$ distance} \\ \midrule
%SigCWGAN  & \textbf{0.4286}  \\
%CWGAN  & 0.4384  \\
%TimeGAN  & 0.4680  \\
%RCGAN  & 0.4466  \\
%GMMN  & 0.4499  \\ \bottomrule
%\end{tabularx}
%\end{table}

%previous table 
%\newcolumntype{Y}{>{\centering\arraybackslash}X}
%\begin{table}[!ht]
%\caption{Numerical results of $\operatorname{VAR}(1)$ for $d = 3$ %with fixed training time of 2 minutes}\label{table_Var_dim=3_time}
%\centering
%\begin{tabularx}{.55\textwidth}{l| Y}
%\toprule
%\multicolumn{1}{l|}{}     & \multicolumn{1}{c}{Temporal %Correlations}  \\ \midrule
%Settings                  & %\multicolumn{1}{c}{$\phi=0.2,\,\,\sigma=0.8$} \\ \midrule
%\multicolumn{2}{c}{Metric on marginal distribution} \\ \midrule
%SigCWGAN  & 0.0314  \\
%CWGAN  & 0.0086  \\
%TimeGAN  & 0.0243  \\
%RCGAN  & 0.0095  \\
%GMMN  & \textbf{0.0084} \\ \midrule
%\multicolumn{2}{c}{Absolute difference of lag-1 autocorrelation} \\ %\midrule
%SigCWGAN  & \textbf{0.0085}  \\
%CWGAN  & 0.0110  \\
%TimeGAN  & 0.0320  \\
%RCGAN  & 0.0332  \\
%GMMN  & 0.0298  \\ \midrule
%\multicolumn{2}{c}{$R^2$ obtained from TSTR. (TRTR first row.)} \\ %\midrule
%\multicolumn{1}{l|}{TRTR} & 0.04197  \\ \midrule
%SigCWGAN  & \textbf{0.0394}  \\
%CWGAN  & 0.0350  \\
%TimeGAN  & 0.0229  \\
%RCGAN  & 0.0214  \\
%GMMN  & 0.0026  \\ \midrule
%\multicolumn{2}{c}{Sig-$W_1$ distance} \\ \midrule
%SigCWGAN  & \textbf{0.4286}  \\
%CWGAN  & 0.4384  \\
%TimeGAN  & 0.4680  \\
%RCGAN  & 0.4466  \\
%GMMN  & 0.4499  \\ \bottomrule
%\end{tabularx}
%\end{table}

\newcolumntype{Y}{>{\centering\arraybackslash}X}
\begin{table}[!ht]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabularx}{1.4\textwidth}{l| Y || Y || Y  || Y}
\toprule
\multicolumn{1}{l|}{Metrics} & \multicolumn{1}{c||}{marginal distribution} &   \multicolumn{1}{c||}{auto-correlation}& 
 \multicolumn{1}{c||}{$R^2(\%)$} & \multicolumn{1}{c}{Sig-$W_1$}    
\\\midrule
SigCWGAN   & 0.0314  &\textbf{0.0085} & \textbf{0.0394} & \textbf{0.4286}  \\\midrule
CWGAN   &0.0086  & 0.0110  & 0.0350  & 0.4384  \\\midrule
TimeGAN   & 0.0243   &  0.0320   & 0.0229  & 0.4680 \\\midrule
RCGAN     & 0.0095   & 0.0332   & 0.0214    & 0.4466  \\\midrule
GMMN      & \textbf{0.0084}   & 0.0298   & 0.0026    & 0.4499   \\\bottomrule
\end{tabularx}}
\caption{Numerical results of $\operatorname{VAR}(1)$ for $d = 3$ with fixed training time of 2 minutes}\label{table_Var_dim=3_time}
\end{table}

